Equivalence of the Empirical Risk Minimization to Regularization on the Family of f-Divergences

The solution to empirical risk minimization with $f$-divergence regularization (ERM-$f$DR) is presented under mild conditions on $f$. Under such conditions, the optimal measure is shown to be unique. Examples of the solution for particular choices of the function $f$ are presented. Previously known solutions to common regularization choices are obtained by leveraging the flexibility of the family of $f$-divergences. These include the unique solutions to empirical risk minimization with relative entropy regularization (Type-I and Type-II). The analysis of the solution unveils the following properties of $f$-divergences when used in the ERM-$f$DR problem: $i\bigl)$ $f$-divergence regularization forces the support of the solution to coincide with the support of the reference measure, which introduces a strong inductive bias that dominates the evidence provided by the training data; and $ii\bigl)$ any $f$-divergence regularization is equivalent to a different $f$-divergence regularization with an appropriate transformation of the empirical risk function.

==> Proof_Lemm_InfDev_Mono_K_fooERM_Type2_v2_IEEEtran.tex <==
% !TEX encoding = UTF-8 Unicode
%-------------------------------------------------%   
%   ___                  _____           
%  / _ \                /  ___|          
% / /_\ \_ __  _ ____  _\ `--.  ___  ___ 
% |  _  | '_ \| '_ \ \/ /`--. \/ _ \/ __|
% | | | | |_) | |_) >  </\__/ /  __/ (__ 
% \_| |_/ .__/| .__/_/\_\____/ \___|\___|
%       | |   | |                        
%       |_|   |_|                      
%-------------------------------------------------%
%<*appxsec>
\section{Proof of Lemma~\ref{lemm_InfDevKfDR}}
%
%</appxsec>

%-------------------------------------------------%
% ______                 __ 
% | ___ \               / _|
% | |_/ / __ ___   ___ | |_ 
% |  __/ '__/ _ \ / _ \|  _|
% | |  | | | (_) | (_) | |  
% \_|  |_|  \___/ \___/|_| 
%-------------------------------------------------%
%<*proof>
\begin{IEEEproof}
\label{AppProofLemmaInfDevKtype2}
%
The properties of the function $N_{Q, \dset{z}}$ in~\eqref{EqType2Krescaling} are proven into two parts.
%
The first part uses the properties of the $f$-divergences regularization to prove it is strictly increasing.
%
The second part proves the continuity of the function $N_{Q, \dset{z}}$ in~\eqref{EqType2Krescaling}.


%-----------------------------------------------------
% 			Part 1 of the Proof
%-----------------------------------------------------
The first part is as follows.
%
For $N_{Q, \dset{z}}$ defined in~\eqref{EqDefNormFunction}, assume that $t \in \set{B}$,  and $\gamma \in \set{A}$ satisfy that
%Under the assumption that the set $\bar{\set{K}}_{Q, \dset{z}}$ in~\eqref{EqDefSetKType2} is not empty, there exists a $t\in \bar{\set{K}}_{Q, \dset{z}}$ and a $\gamma \in \reals$, such that
%
\begin{equation}
\label{EqProofKrescalingL1}
N_{Q, \dset{z}}(t) = \gamma,
\end{equation}
%
which implies that
%
\begin{subequations}
\label{Eq_ProofLambdaIsTheInvOfKbar}
\begin{IEEEeqnarray}{rCl}
	1 
	& = & \int \frac{\diff \Pgibbs[\dset{z}][t]{P}{Q}}{\diff Q}(\thetav) \diff Q(\thetav)
	\label{Eq_ProofLambdaIsTheInvOfKbar_s1}\\
	& = & \int \dot{f}^{-1}(-\frac{t + \foo{L}_{\dset{z}}(\thetav)}{\gamma})\diff Q(\thetav),
	\label{Eq_ProofLambdaIsTheInvOfKbar_s2}
\end{IEEEeqnarray}
\end{subequations}
%
with $\set{B}$ and $\set{A}$ defined in~\eqref{EqDefSetB} and~\eqref{EqDefMapNormFunction}, respectively.
%
%Note that from the fact that $\dot{f}^{-1}$ is strictly increasing, it holds that for all $t \in \set{B}$ and for all $\thetav \in \supp Q$, it holds that
%
Note that the inverse $\dot{f}^{-1}$ exists from the fact that $f$ is strictly convex, which implies that $\dot{f}$ is a strictly increasing function. Hence, $\dot{f}^{-1}$ is also a strictly increasing function in $\set{B}$ \cite[Theorem 5.6.9]{bartle2000introduction}.
%
Moreover, from the assumption that $f$ is strictly convex and differentiable, it holds that $\dot{f}$ is continuous \cite[Proposition $5.44$]{douchet2010Analyse}. This implies that $\dot{f}^{-1}$ is continuous.

%
%
%
%where $N_{Q, \dset{z}}$ is defined in~\eqref{EqType2Krescaling}.
%
%Let the set $\set{I}$ be $\set{I} = \{N_{Q, \dset{z}}(\alpha) \in \reals : \alpha \in \bar{\set{K}}_{Q, \dset{z}}\}$  for which a solution exists$\set{I} \subseteq \reals$, and let the function $N_{Q, \dset{z}}:\set{I} \rightarrow (0, \infty)$ be the functional inverse of $N_{Q, \dset{z}}$ in~\eqref{EqType2Krescaling} given by
%Let the function $N_{Q, \dset{z}}:\set{A} \rightarrow (0, \infty)$ be the functional inverse of $N_{Q, \dset{z}}$ in~\eqref{EqType2Krescaling} given by
%%
%\begin{IEEEeqnarray}{rCl}
%\label{EqDefNormFunction}
%	N_{Q, \dset{z}}(\gamma) 
%	& = & \frac{1}{\int \frac{1}{\foo{L}_{\dset{z}}(\thetav) + \gamma}\diff Q(\thetav)},
%\end{IEEEeqnarray}
%%
%which follows from the constraint in~\eqref{Eq_ProofLambdaIsTheInvOfKbar} and the equality in~\eqref{EqProofKrescalingL1}. %The definition of $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction} completes the first part of the proof.

From~\eqref{Eq_ProofLambdaIsTheInvOfKbar} and the fact that $\dot{f}^{-1}$ is continuous, if $t \in \set{B}$, then it holds that
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarNoLambdaIsFinite}	
	0 < \int \dot{f}^{-1}(- t -\foo{L}_{\dset{z}}(\thetav))\diff Q(\thetav)
	& < & \infty.
\end{IEEEeqnarray}
%
%which implies that for all $\gamma \in \set{A}$, with $\set{A}$ in~\eqref{EqDefMapNormFunction}, the function $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction}~satisfies
%%
%\begin{IEEEeqnarray}{rCl}
% \infty > N_{Q, \dset{z}}(\gamma) & > & 0.
%\end{IEEEeqnarray}
%
From~\eqref{Eq_ProofKbarNoLambdaIsFinite} and the fact that $\dot{f}^{-1}$ is strictly increasing, for all $(t_1, t_2) \in \set{B}^2$, such that $t_1<t_2
$, for all $\thetav \in \supp Q$, it holds that
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarNoLambdaIsGam1vs2Singular}	
	 \dot{f}^{-1}(- t_1-\foo{L}_{\dset{z}}(\thetav))
	& > &  \dot{f}^{-1}(- t_2-\foo{L}_{\dset{z}}(\thetav)),
\end{IEEEeqnarray}
%
which implies that
%
\begin{equation}
\label{Eq_ProofKbarNoLambdaIsGam1vs2}	
	\int \dot{f}^{-1}(- t_1-\foo{L}_{\dset{z}}(\thetav))\diff Q(\thetav)
	 >  \int \dot{f}^{-1}(- t_2-\foo{L}_{\dset{z}}(\thetav))\diff Q(\thetav).
\end{equation}
%
Therefore, from equality~\eqref{Eq_ProofLambdaIsTheInvOfKbar} and inequality~\eqref{Eq_ProofKbarNoLambdaIsGam1vs2} for all $(t_1, t_2) \in \set{B}^2$, such that $t_1<t_2$, the function $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction}~satisfies
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarStricIncreaseGam1vs2}
N_{Q, \dset{z}}(\gamma_1)  & < & 	N_{Q, \dset{z}}(\gamma_2),
\end{IEEEeqnarray}
%
which implies that the function $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction} is strictly increasing. Furthermore, from inequality~\eqref{Eq_ProofKbarStricIncreaseGam1vs2} and the fact that $\Pgibbs[\dset{z}][t]{P}{Q}$ is unique (see Theorem~\ref{Theo_f_ERMRadNik}), it follows that $N_{Q, \dset{z}}$ is bijective, which completes the proof of the first part. 

%-----------------------------------------------------
% 			Part 2 of the Proof
%-----------------------------------------------------
The second part is as follows.
%
The continuity of the function $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction} is shown by considering an arbitrary $\epsilon > 0$ and a pair $(\gamma_1, \gamma_2) \in \set{A}^2$ under the condition
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarContEpsDelt}
\epsilon & > & \abs{N_{Q, \dset{z}}(\gamma_2) - N_{Q, \dset{z}}(\gamma_1)}.
\end{IEEEeqnarray}
%
%Then, from the fact that $N_{Q, \dset{z}}$ is bijective and strictly increasing let $\gamma_1 < \gamma_2$ without loss of generality, inequality~\eqref{Eq_ProofKbarContEpsDelt} can be equivalently expressed as
From the fact that $N_{Q, \dset{z}}$ is bijective and strictly increasing, let the pair $\gamma_1$, and $\gamma_2$ satisfy $\gamma_1 < \gamma_2$, without loss of generality. Thus, it holds that
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarContEpsDeltNoAbs}
 \abs{N_{Q, \dset{z}}(\gamma_2) - N_{Q, \dset{z}}(\gamma_1)}
& = & N_{Q, \dset{z}}(\gamma_2) - N_{Q, \dset{z}}(\gamma_1).
\end{IEEEeqnarray}
%
Substituting equality~\eqref{Eq_ProofKbarContEpsDeltNoAbs} into~\eqref{Eq_ProofKbarContEpsDelt} yields
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarContEpsDeltNoAbs2}
N_{Q, \dset{z}}(\gamma_1) + \epsilon & > & N_{Q, \dset{z}}(\gamma_2) .
\end{IEEEeqnarray}
%
From the fact that $N_{Q, \dset{z}}$ is bijective, evaluating inequality~\eqref{Eq_ProofKbarContEpsDeltNoAbs2} with $N_{Q, \dset{z}}$ in~\eqref{EqDefMapNormFunction} leads to
%
\begin{subequations}
\label{Eq_ProofKbarInvEpsDeltNoAbs}
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarInvEpsDeltNoAbs_s1}
N^{-1}_{Q, \dset{z}}(N_{Q, \dset{z}}(\gamma_1) + \epsilon) 
	& > & N^{-1}_{Q, \dset{z}}(N_{Q, \dset{z}}(\gamma_2))\\
	& = & \gamma_2.\label{Eq_ProofKbarInvEpsDeltNoAbs_s2}
\end{IEEEeqnarray}
\end{subequations}
%
Subtracting $\gamma_1$ from both sides in~\eqref{Eq_ProofKbarInvEpsDeltNoAbs}, results in
%
\begin{subequations}
\label{Eq_ProofKbarInvEpsDeltNoAbs2}
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarInvEpsDeltNoAbs2_s1}
N^{-1}_{Q, \dset{z}}(N_{Q, \dset{z}}(\gamma_1) + \epsilon)  - \gamma_1
	& > & \gamma_2 - \gamma_1\\
	& = & \abs{\gamma_2 - \gamma_1},	\label{Eq_ProofKbarInvEpsDeltNoAbs2_s2}
\end{IEEEeqnarray}
\end{subequations}
%
where equality~\eqref{Eq_ProofKbarInvEpsDeltNoAbs2_s2} follows from the condition that $\gamma_2 > \gamma_1$.
%
Thus, from~\eqref{Eq_ProofKbarInvEpsDeltNoAbs2} it follows that for all $\epsilon > 0$, there exist a $\delta > 0$ that satisfies
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofKbarInvDeltafunction}
\delta & = & N^{-1}_{Q, \dset{z}}(N_{Q, \dset{z}}(\gamma_1) + \epsilon) - \gamma_1 ,
\end{IEEEeqnarray}
%
which implies the function $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction} is continuous for all $\gamma \in \set{A}$.
%
From~\eqref{Eq_ProofKbarInvDeltafunction} the function $N_{Q, \dset{z}}$ is continuous and strictly increasing, which completes the proof.
%
%If for all $\delta \in (t^{\star}_{Q, \dset{z}}, \infty)$, it holds that $ \delta -t^{\star}_{Q, \dset{z}} < Q(\set{L}(\delta))$, taking the limit as $\delta$ approaches $t^{\star}_{Q, \dset{z}}$, yields
%\begin{IEEEeqnarray}{rCl}
%%\IEEEeqnarraymulticol{3}{l}{%
%\int \frac{1}{\foo{L}_{\dset{z}}(\thetav) - \delta^\star_{Q, \dset{z}}}\diff Q(\thetav)
%%}\nonumber\\ \qquad
%& \geq & \lim_{\delta \rightarrow t^{\star}_{Q, \dset{z}}} \frac{Q(\set{L}_{\dset{z}}(\delta))}{( \delta  - \delta^\star_{Q, \dset{z}})}\\
%& = & \infty,
%\end{IEEEeqnarray}
% which contradicts~\eqref{Eq_ProofLambdaIsTheInvOfKbar_s1}.
%
%From the contradictions induced by~\eqref{EqProofT2Contradict1} and~\eqref{EqProofT2lowBoundDowndDelta}, it implies that for all $\alpha \in (0, \infty)$, it holds that $N_{Q, \dset{z}}(\alpha) \in (-\delta^\star_{Q, \dset{z}}, \infty)$.
%%
%Hence, the functional inverse $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction} is well defined for $N_{Q, \dset{z}}:(-\delta^\star_{Q, \dset{z}}, \infty)\rightarrow (0, \infty)$.
\end{IEEEproof}
%</proof>
%-------------------------------------------------%
%
% ███████╗███╗░░██╗██████╗░
% ██╔════╝████╗░██║██╔══██╗
% █████╗░░██╔██╗██║██║░░██║
% ██╔══╝░░██║╚████║██║░░██║
% ███████╗██║░╚███║██████╔╝
% ╚══════╝╚═╝░░╚══╝╚═════╝░

%-------------------------------------------------%
%  _
% | |                                   
% | |     ___ _ __ ___  _ __ ___   __ _ 
% | |    / _ \ '_ ` _ \| '_ ` _ \ / _` |
% | |___|  __/ | | | | | | | | | | (_| |
% \_____/\___|_| |_| |_|_| |_| |_|\__,_|
%
%-------------------------------------------------%
%        Lemma Type-II Function
%-------------------------------------------------%
%\begin{lemma}
%\label{lemm_InfDevKfDR}
%Given a fixed probability measure $Q$ and a dataset $\dset{z}$, the function $N_{Q, \dset{z}}$ in~\eqref{EqType2Krescaling} is positive monotonically increasing, continuous, and differentiable infinitely many times in $\lambda\, \in~  \infty)$.
%\end{lemma}
%%
%\begin{IEEEproof}
%		The proof is presented in Appendix~\ref{AppProofLemmaInfDevKtype2}.
%\end{IEEEproof}
%-------------------------------------------------%


==> Proof_Lemm_NoMinF_nneg_IEEEtran.tex <==
% !TEX encoding = UTF-8 Unicode
%-------------------------------------------------%   
%   ___                  _____           
%  / _ \                /  ___|          
% / /_\ \_ __  _ ____  _\ `--.  ___  ___ 
% |  _  | '_ \| '_ \ \/ /`--. \/ _ \/ __|
% | | | | |_) | |_) >  </\__/ /  __/ (__ 
% \_| |_/ .__/| .__/_/\_\____/ \___|\___|
%       | |   | |                        
%       |_|   |_|                      
%-------------------------------------------------%
%<*appxsec>
\section{Proof of Lemma~\ref{lemm_fDR_No_minRegF_nneg}}\label{app_proof_lemm_fDR_No_minRegF_nneg}
%
%</appxsec>

%-------------------------------------------------%
% ______                 __ 
% | ___ \               / _|
% | |_/ / __ ___   ___ | |_ 
% |  __/ '__/ _ \ / _ \|  _|
% | |  | | | (_) | (_) | |  
% \_|  |_|  \___/ \___/|_| 
%-------------------------------------------------%
%<*proof>
\begin{IEEEproof}
\label{proof_lemm_fDR_No_minRegF_nneg}
	The following proof by contradiction is divided into three parts. In the first part, an auxiliary function is introduced and proven to be continuous. In the second part, a contradiction is shown under the assumption that $\dot{f}^{-1}$ is nonnegative and the continuity of the auxiliary. Finally, it is shown that for nonnegative $\dot{f}^{-1}$, the set of admissible regularization factors is the positive reals.

%To study the $\set{B}$ in~\eqref{EqDefSetB} for functions $f$ that induce nonnegative $\dot{f}^{-1}$, 
The first part is as follows.
%
Let the function $k: \set{B} \to (0, +\infty)$ be such that
\begin{IEEEeqnarray}{rcl}
\label{EqkWA}
k(t) & = &  \int \dot{f}^{-1}(\frac{-t - \foo{L}_{\dset{z}}(\thetav)}{\lambda} ) \diff Q (\vect{\theta}).
\end{IEEEeqnarray}
%
The first step is to prove that the function $k$ in \eqref{EqkWA} is continuous in $\set{B}$. This is proved by showing that $k$ always exhibits a limit. 
%
Note that from the fact that $\dot{f}^{-1}$ is strictly increasing, it holds that for all $t \in \set{B}$ and for all $\vect{\theta} \in \supp Q$, it holds that 
\begin{IEEEeqnarray}{rcl}
\label{EqThoseEyesISawToday}
 \dot{f}^{-1}(\frac{-t - \foo{L}_{\dset{z}}(\thetav)}{\lambda}) & \leq  & \dot{f}^{-1}(-\frac{t}{\lambda}), \end{IEEEeqnarray}
where equality holds if and only if $ \foo{L}_{\dset{z}}(\thetav)  = 0$.
%
Now, from the fact that $\dot{f}^{-1}$ is continuous it follows that for all $a \in \set{B}$, it holds that
%
\begin{IEEEeqnarray}{rcl}
\label{EqSuchABeautiflFace}
\lim_{t \to a} \dot{f}^{-1}(\frac{-t - \foo{L}_{\dset{z}}(\thetav)}{\lambda}) & = &  \dot{f}^{-1}(\frac{-a - \foo{L}_{\dset{z}}(\thetav)}{\lambda}).
\end{IEEEeqnarray}
%
Hence, from the dominated convergence theorem \cite[Theorem~$1.6.9$]{ash2000probability}, the following limit exists and satisfies  
\begin{IEEEeqnarray}{rcl}
\label{EqSuchACrazyDay}
\lim_{t \to a} k(t) & = & \lim_{t \to a}  \int \dot{f}^{-1}(\frac{-t - \foo{L}_{\dset{z}}(\thetav)}{\lambda} ) \diff Q (\vect{\theta})\\
 & = &  \int  (\lim_{t \to a} \dot{f}^{-1}(\frac{-t   - \foo{L}_{\dset{z}}(\thetav)}{\lambda} ) )\diff Q (\vect{\theta})\\
 & = & \int  \dot{f}^{-1}(\frac{-a - \foo{L}_{\dset{z}}(\thetav)}{\lambda}  )\diff Q (\vect{\theta})\\
 & = & k(a),
\end{IEEEeqnarray}
which proves that the function $k$ in \eqref{EqkWA} is continuous.
%

The second part is as follows. Under the assumption that $f$ induces a nonnegative $\dot{f}^{-1}$ and that $\set{B}$ is nonempty, from Lemma~\ref{lemm_fDR_kset} the set $\set{B}$ is either $[t^{\star}_{Q,\dset{z}},\infty)$ or $(t^{\star}_{Q,\dset{z}},\infty)$. Hence, it is sufficient to show that assuming $\set{B}$ is equal to $[t^{\star}_{Q,\dset{z}},\infty)$ and $\dot{f}^{-1}$ is nonnegative leads to a contradiction. From Lemma~\ref{lemm_fDR_kset} it follows that 
%
\begin{IEEEeqnarray}{rCl}
	k(t^{\star}_{Q,\dset{z}}) < \infty,
\end{IEEEeqnarray}
%
with the function $k$ in~\eqref{EqkWA} and $t^{\star}_{Q,\dset{z}}$ defined in~\eqref{EqDefTStar}.
%
Thus, from the fact that $k$ in \eqref{EqkWA} is continuous, for $t <t^{\star}_{Q,\dset{z}}$, it follows that $k(t) < \infty$, which implies there exists a set $C = \{\thetav \in \supp Q: \dot{f}^{-1}(\frac{-t - \foo{L}_{\dset{z}}(\thetav)}{\lambda}) < 0\}$ such that $t \not\in \set{B}$. However, this contradicts the assumption that $\dot{f}^{-1}$ is nonnegative, which implies that $\set{B} = (t^{\star}_{Q,\dset{z}},\infty)$. This completes the second part of the proof.

The third part is as follows.
%
%Observe that the function
From the fact that $\set{B}$ is nonempty, there is a $t \in \set{B}$ and a $\lambda \in (0,\infty)$ such that,
%
\begin{IEEEeqnarray}{rCl}
	1 = \int \dot{f}^{-1}(-\frac{t+\foo{L}_{\dset{z}}}{\lambda}) \diff Q(\thetav).
\end{IEEEeqnarray}
% 
From the fact that the function $\dot{f}^{-1}$ is continuous and strictly increasing, for all $t_1 \in (t^{\star}_{Q,\dset{z}},t)$ and for all $t_2 \in (t,\infty)$, it holds that
\begin{equation}
\label{EqfDRforTs}
	\int \dot{f}^{-1}(-\frac{t_1+\foo{L}_{\dset{z}}}{\lambda}) \diff Q(\thetav)  >  1 
	>  \int \dot{f}^{-1}(-\frac{t_2+\foo{L}_{\dset{z}}}{\lambda}) \diff Q(\thetav).
\end{equation}
%
Under the same argument, for all $\lambda_1 \in (0,\lambda)$ and for all $\lambda_2 \in (\lambda,\infty)$, it holds that
%
%\begin{IEEEeqnarray}{rCl}
%	\int \dot{f}^{-1}(-\frac{t+\foo{L}_{\dset{z}}}{\lambda_1}) \diff Q(\thetav) & > & 1 \\
%	& > & \int \dot{f}^{-1}(-\frac{t+\foo{L}_{\dset{z}}}{\lambda_2}) \diff Q(\thetav).
%\end{IEEEeqnarray}
\begin{equation}
\label{EqfDRforLambdas}
	\int \dot{f}^{-1}(-\frac{t+\foo{L}_{\dset{z}}}{\lambda_1}) \diff Q(\thetav)  >  1 
	>  \int \dot{f}^{-1}(-\frac{t+\foo{L}_{\dset{z}}}{\lambda_2}) \diff Q(\thetav).
\end{equation}

Hence, given that the function $k$ in \eqref{EqkWA} is continuous, strictly decreasing, from \eqref{EqfDRforTs} then, there always exists two reals $t_1$ and $t_2$ in $\set{B}$ such that $k(t_1) < 1 < k(t_2)$, it follows from the intermediate-value theorem \cite[Theorem~$4.23$]{rudin1953bookPrinciples} that there always exists a unique real $t \in \set{B}$ such that $k(t) = 1$. Furthermore, for all $t \in \set{B}$ there always exists two reals $\lambda_1$ and $\lambda_2$ in $(0,\infty)$ such that inequality \eqref{EqfDRforLambdas} holds, it follows from the intermediate-value theorem \cite[Theorem~$4.23$]{rudin1953bookPrinciples} that there always exists a unique real $t \in \set{B}$ for all $\lambda \in (0,\infty)$ such that $k(t) = 1$. 
Finally, from the fact that $N_{Q,\dset{z}}$ in \eqref{EqDefNormFunction} is continuous and strictly increasing, if $\set{B} = (t^{\star}_{Q,\dset{z}},\infty)$ then the set of admisible regularization factors $\set{A}$ in \eqref{EqDefMapNormFunction} is identical to $(0,\infty)$, which completes the proof.
%Note also that such a function $k$ is strictly decreasing, from the fact that $\dot{f}^{-1}$ is strictly increasing in $\set{A}$. 
%
%The proof continues by assuming that there exists a pair $(t_1, t_2) \in \set{B}^2$, such that $k(t_1) < 1 < k(t_2)$.
%%
%Consider the set $\set{C}_{t_1} 
%%= \left\lbrace \vect{\theta} \in \set{M} : \dot{f} (1) \leqslant \left( \frac{- t_1 -  \mathsf{L}_{\vect{z}} (\vect{\theta} )}{\lambda}\right)  \right\rbrace 
%= \left\lbrace \vect{\theta} \in \set{M} : \dot{f}^{-1}  \left( \frac{- t_1 - \mathsf{L}_{\vect{z}} (\vect{\theta} )}{\lambda}\right) \geqslant 1 \right\rbrace$.
%%
%Assume that $1 < k(t_1)$. Hence, 
%\begin{IEEEeqnarray}{rcl}
%1 & < & k(t_1)\\
%& = & \int_{\set{C}_{t_1}} \dot{f}^{-1}(-\frac{t_1 + \foo{L}_{\dset{z}}(\thetav)}{\lambda}) \diff Q(\thetav) + \int_{\set{M} \setminus \set{C}_{t_1}} \dot{f}^{-1}(-\frac{t_1 + \foo{L}_{\dset{z}}(\thetav)}{\lambda}) \diff Q(\thetav)\\
%& < & \int_{\set{C}_{t_1}} \dot{f}^{-1}(-\frac{t_1 + \foo{L}_{\dset{z}}(\thetav)}{\lambda}) \diff Q(\thetav) + \int_{\set{M} \setminus \set{C}_{t_1}}   \diff Q(\thetav)\\
%& \leqslant & \int_{\set{C}_{t_1}} \dot{f}^{-1}(-\frac{t_1 + \underline{\gamma}_{\dset{z}} }{\lambda}) \diff Q(\thetav) + \int_{\set{M} \setminus \set{C}_{t_1}}  \diff Q(\thetav)\\
%& \leqslant & Q\left( \set{C}_{t_1} \right) \dot{f}^{-1}(-\frac{t_1 + \underline{\gamma}_{\dset{z}}}{\lambda}) + 1 -  Q\left( \set{C}_{t_1} \right),
%\label{EqInsommia97}
%\end{IEEEeqnarray}
%where $\underline{\gamma}_{\dset{z}}$ is defined in \eqref{EqLunderline}. 
%%
%The inequalities in \eqref{EqInsommia97} imply that $t_1$ must satify $\dot{f}^{-1}(-\frac{t_1 + \underline{\gamma}_{\dset{z}}}{\lambda}) > 1$. This is the same as requiring that 
%\begin{IEEEeqnarray}{rcl}
%\label{Eqfdot_one_t1_ineq}
%\dot{f}(1) & < & -\frac{t_1+ \underline{\gamma}_{\dset{z}}}{\lambda},
%\end{IEEEeqnarray}
%as a consequence of the function $\dot{f}$ being strictly increasing.
%%
%%Note that from the subset of $\set{B}$ defined in \eqref{EqDecreusefondSetB}
%% and \eqref{Eqfdot_one_t1_ineq}, the assumption that the real value $t_1 \in \set{B}$ holds if and only if,
%%
%From the inequality \eqref{Eqfdot_one_t1_ineq}, it holds that $\lambda\dot{f}(1)  <  -t_1 - \underline{\gamma}_{\dset{z}}$, which implies that
%%
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t1_ineq_condition_s1}
%	t_1 & < & -\lambda \dot{f}(1) - \underline{\gamma}_{\dset{z}}.\label{Eq_t1_ineq_condition_s2}
%\end{IEEEeqnarray}
%%
%To show that there exists a $t_1 \in \set{B}$, such that $1<k(t_1)$, the intersection between the set $ \left(- \lambda a_2 - \underline{\gamma}_{\vect{z}} , -\lambda a_1 - \bar{\gamma}_{\vect{z}}  \right)$ in \eqref{EqDecreusefondSetB} and the interval $\left( -\infty , -\lambda \dot{f}(1) - \underline{\gamma}_{\dset{z}} \right)$ must be not empty. This is the same as requiring that 
%%
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t1_ineq_withBc1Hell}
%	-\lambda a_2 -\underline{\gamma}_{\dset{z}} & <   -\lambda \dot{f}(1) -\underline{\gamma}_{\dset{z}} < &-\lambda a_1 -\bar{\gamma}_{\dset{z}}. 
%\end{IEEEeqnarray}
%%
%The inequality $-\lambda a_2 -\underline{\gamma}_{\dset{z}} <  -\lambda \dot{f}(1) -\underline{\gamma}_{\dset{z}}$  is always satisfied as a consequence of the fact that %
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t1_ineq_case1}
% \dot{f}(1) & < & a_2.
% \end{IEEEeqnarray}
%%
%%
%The inequality $-\lambda \dot{f}(1) -\underline{\gamma}_{\dset{z}} < -\lambda a_1 -\bar{\gamma}_{\dset{z}}$ implies
%%
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t1_ineq_withBc2}
%%	-\lambda a_1 -\bar{\gamma}_{\dset{z}} 	& >  & -\lambda \dot{f}(1) -\underline{\gamma}_{\dset{z}}\\
%	 -\lambda (a_1- \dot{f}(1)) & >  & \bar{\gamma}_{\dset{z}} -\underline{\gamma}_{\dset{z}}\\
%	 \lambda (\dot{f}(1)-a_1) & >  & \bar{\gamma}_{\dset{z}}-\underline{\gamma}_{\dset{z}}\\
%	 \lambda & >  &  \frac{\bar{\gamma}_{\dset{z}}-\underline{\gamma}_{\dset{z}}}{\dot{f}(1)-a_1},\label{Eq_t1_ineq_withBc2_s4}
%\end{IEEEeqnarray}
%% 
%which occurs under the assumption in \eqref{EqTheFinalAssumption} of the theorem. Hence, there always exists a real $t_1$ in $\set{B}$ such that $1 < k(t_1)$.
%
%Assume now that $1 > k(t_2)$. Hence, 
%\begin{IEEEeqnarray}{rcl}
%1 & > & k(t_2)\\
%& = & \int_{\set{C}_{t_2}} \dot{f}^{-1}(-\frac{t_2 + \foo{L}_{\dset{z}}(\thetav)}{\lambda}) \diff Q(\thetav) + \int_{\set{M} \setminus \set{C}_{t_2}} \dot{f}^{-1}(-\frac{t_2 + \foo{L}_{\dset{z}}(\thetav)}{\lambda}) \diff Q(\thetav)\\
%& \geqslant & \int_{\set{C}_{t_2}}  \diff Q(\thetav) + \int_{\set{M} \setminus \set{C}_{t_2}} \dot{f}^{-1}(-\frac{t_2 + \foo{L}_{\dset{z}}(\thetav)}{\lambda})  \diff Q(\thetav)\\
%& \geqslant & \int_{\set{C}_{t_2}}  \diff Q(\thetav) + \int_{\set{M} \setminus \set{C}_{t_2}} \dot{f}^{-1}(-\frac{t_2 + \bar{\gamma}_{\dset{z}}}{\lambda})  \diff Q(\thetav)\\
%\label{EqSleepingBigTime06}
%& = & Q\left( \set{C}_{t_2} \right)  + \left(1 -  Q\left( \set{C}_{t_2} \right)  \right) \dot{f}^{-1}(-\frac{t_2 + \bar{\gamma}_{\dset{z}}}{\lambda}),
%\end{IEEEeqnarray}
%where $\bar{\gamma}_{\dset{z}}$ is defined in \eqref{EqLbar}. 
%%
%The inequalities in \eqref{EqSleepingBigTime06} imply that $t_2$ must satify $\dot{f}^{-1}(-\frac{t_2 + \bar{\gamma}_{\dset{z}}}{\lambda}) < 1$. This is the same as requiring that 
%\begin{IEEEeqnarray}{rcl}
%\label{Eqfdot_one_t2_ineq}
%\dot{f}(1) & > & -\frac{t_2 + \bar{\gamma}_{\dset{z}}}{\lambda},
%\end{IEEEeqnarray}
%as a consequence of the function $\dot{f}$ being monotonically increasing. 
%%
%The inequality in \eqref{Eqfdot_one_t2_ineq}, implies $\lambda\dot{f}(1)  >  -t_2 - \bar{\gamma}_{\dset{z}}$, which is the same as requiring that 
%%
%\begin{subequations}
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t2_ineq_condition_s2}
%	t_2 & > & -\lambda \dot{f}(1) - \bar{\gamma}_{\dset{z}}.
%\end{IEEEeqnarray}
%\end{subequations}
%%
%To show that the $t_2$ in \eqref{EqSleepingBigTime06} satisfies $t_2 \in \set{B}$, the intersection between the set $ \left(- \lambda a_2 - \underline{\gamma}_{\vect{z}} , -\lambda a_1 - \bar{\gamma}_{\vect{z}}  \right)$ in \eqref{EqDecreusefondSetB} and the interval $\left( -\lambda \dot{f}(1) - \bar{\gamma}_{\dset{z}}, +\infty \right)$ must be not empty. This is the same as requiring that 
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t1_ineq_withBc1HellLate}
%	-\lambda a_2 -\underline{\gamma}_{\dset{z}} & <   -\lambda \dot{f}(1) -\bar{\gamma}_{\dset{z}} < &-\lambda a_1 -\bar{\gamma}_{\dset{z}}. 
%\end{IEEEeqnarray}
%%
%The inequality $  -\lambda \dot{f}(1) -\bar{\gamma}_{\dset{z}} < -\lambda a_1 -\bar{\gamma}_{\dset{z}}$ is always satisfied as a consequence of the fact that
%%
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t2_ineq_case1}
%	 \dot{f}(1) & > & a_1. 
%\end{IEEEeqnarray}
%%
%The inequality $-\lambda a_2 -\underline{\gamma}_{\dset{z}}  <   -\lambda \dot{f}(1) -\bar{\gamma}_{\dset{z}}$ implies
%%
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_t2_ineq_withBc2}
%%	-\lambda \dot{f}(1) -\bar{\gamma}_{\dset{z}} & > & -\lambda a_2 -\underline{\gamma}_{\dset{z}}\\
%	 \lambda (a_2 - \dot{f}(1)) & >  & \bar{\gamma}_{\dset{z}}-\underline{\gamma}_{\dset{z}}\\
%	 \lambda & >  &  \frac{\bar{\gamma}_{\dset{z}}-\underline{\gamma}}{a_2 - \dot{f}(1)}.\label{Eq_t2_ineq_withBc2_s4}
%\end{IEEEeqnarray}
%%
%which occurs under the assumption in \eqref{EqTheFinalAssumption} of the theorem. Hence, there always exists a real $t_2$ in $\set{B}$ such that $1 > k(t_2)$.
%
%
%It has already been established that $f(1) = 0$, the function $f$ is continuous and differentiable. Hence, $\dot{f}(1)$ is well defined. Thus, from \eqref{Eq_t1_ineq_withBc2_s4} and \eqref{Eq_t2_ineq_withBc2_s4}, there exists a pair $(t_1, t_2) \in \set{B}^2$, such that $k(t_1) < 1 < k(t_2)$, if
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_lambda_ineq_withB2}
%	\lambda > \max\{\frac{\bar{\gamma}_{\dset{z}}-\underline{\gamma}_{\dset{z}}}{\dot{f}(1)-a_1},\frac{\bar{\gamma}_{\dset{z}}-\underline{\gamma}_{\dset{z}}}{a_2-\dot{f}(1)}\}.
%\end{IEEEeqnarray}
%
%%\begin{IEEEeqnarray}{rcl}
%%\label{EqApremMagique}
%%-\frac{t_2 + \bar{\gamma}_{\dset{z}}}{\lambda} &  < \dot{f}(1)  < & -\frac{t_1+ \underline{\gamma}_{\dset{z}}}{\lambda}.
%%\end{IEEEeqnarray}
%%%
%%Note that by choosing $t_1$ and $t_2$ from $\set{B}$ in \eqref{EqDecreusefondSetB} such that
%%\begin{IEEEeqnarray}{rcl}
%%- \lambda a_2 - \underline{\gamma}_{\vect{z}} < t_1 <  t_2  <  -\lambda a_1 - \bar{\gamma}_{\vect{z}},
%%\end{IEEEeqnarray}
%%it holds from \eqref{EqApremMagique} that
%%\begin{IEEEeqnarray}{rcl}
%% a_1 < -\frac{t_2 + \bar{\gamma}_{\dset{z}}}{\lambda} &  < \dot{f}(1)  < & -\frac{t_1+ \underline{\gamma}_{\dset{z}}}{\lambda} = a_2,
%%\end{IEEEeqnarray}
%%which is always verified.
%%
%Hence, given that the function $k$ in \eqref{EqkWA} is continuous, strictly decreasing, and if the regularization factor $\lambda$ satisfies \eqref{Eq_lambda_ineq_withB2}, then, there always exists two reals $t_1$ and $t_2$ in $\set{B}$ such that $k(t_1) < 1 < k(t_2)$, it follows from the intermediate-value theorem \cite[Theorem~$4.23$]{rudin1953bookPrinciples} that there always exists a unique real $t \in \set{B}$ such that $k(t) = 1$.
%%
%
%Finally, note that the objective function in~\eqref{EqOpProblemType2fproof9876} is the sum of two terms. 
%	%
%	The first one, i.e., $ \int \foo{L}_{\dset{z}}( \thetav )g( \thetav )  \diff Q ( \thetav )$, is linear with $g$.
%	%
%	The second, i.e., $\int f (g(\thetav)) \diff Q(\thetav)$, is strictly convex with  $g$ from the assumption that $f$ is strictly convex.
%	%
%	Hence, given that $\lambda>0$, the sum of both terms is strictly convex with  $g$.  This implies the uniqueness of $\Pgibbs{P}{Q}$.
%--------------------------------------------------End
\end{IEEEproof}
%</proof>
%-----------------------------------------------------
%
% ███████╗███╗░░██╗██████╗░
% ██╔════╝████╗░██║██╔══██╗
% █████╗░░██╔██╗██║██║░░██║
% ██╔══╝░░██║╚████║██║░░██║
% ███████╗██║░╚███║██████╔╝
% ╚══════╝╚═╝░░╚══╝╚═════╝░


%-------------------------------------------------%
%  _
% | |                                   
% | |     ___ _ __ ___  _ __ ___   __ _ 
% | |    / _ \ '_ ` _ \| '_ ` _ \ / _` |
% | |___|  __/ | | | | | | | | | | (_| |
% \_____/\___|_| |_| |_|_| |_| |_|\__,_|
%
%-------------------------------------------------%


==> Proof_Lemm_minRegFactor_IEEEtran.tex <==
% !TEX encoding = UTF-8 Unicode
%-------------------------------------------------%   
%   ___                  _____           
%  / _ \                /  ___|          
% / /_\ \_ __  _ ____  _\ `--.  ___  ___ 
% |  _  | '_ \| '_ \ \/ /`--. \/ _ \/ __|
% | | | | |_) | |_) >  </\__/ /  __/ (__ 
% \_| |_/ .__/| .__/_/\_\____/ \___|\___|
%       | |   | |                        
%       |_|   |_|                      
%-------------------------------------------------%
%<*appxsec>
\section{Proof of Lemma~\ref{lemm_fDR_kset}}\label{app_proof_lemm_fDR_kset}
%
%</appxsec>

%-------------------------------------------------%
% ______                 __ 
% | ___ \               / _|
% | |_/ / __ ___   ___ | |_ 
% |  __/ '__/ _ \ / _ \|  _|
% | |  | | | (_) | (_) | |  
% \_|  |_|  \___/ \___/|_| 
%-------------------------------------------------%
%<*proof>
\begin{IEEEproof}
\label{proof_lemm_fDR_kset}
%-----------------------------------------------------
% 			Part 3 of the Proof
%-----------------------------------------------------
%The third part is as follows.
%
The proof shows that if $\set{B}$ in~\eqref{EqDefSetB} is not empty, then the domain of the function $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction} is an interval of $\reals$. The proof is divided into two parts, in the first part it is shown that $\set{B}$ is always open from the right. The second part uses $t^{\star}_{Q, \dset{z}}$ the set from the left.

The first part is as follows.
%
From Lemma~\ref{lemm_InfDevKfDR}, if there exists a $t_1 \in \set{B}$, then it holds
%
\begin{IEEEeqnarray}{rCl}
\label{Eq_ProofSetBNoLambdaIsFinite}	
	0 < \int \dot{f}^{-1}(- t_1 - \foo{L}_{\dset{z}}(\thetav))\diff Q(\thetav)
	& < & \infty.
\end{IEEEeqnarray}
%
From~\eqref{Eq_ProofSetBNoLambdaIsFinite} and the fact that $N_{Q, \dset{z}}$ is strictly increasing, for all $t \in \{s \in \reals : s \geq t_1\}$, it holds that
%
\begin{equation}
%\IEEEeqnarraymulticol{3}{l}{
\label{Eq_ProofSetBintegralbounded}	
	\int \dot{f}^{-1}(- t_1 -\foo{L}_{\dset{z}}(\thetav))\diff Q(\thetav)
	 >   \int \dot{f}^{-1}(- t -\foo{L}_{\dset{z}}(\thetav))\diff Q(\thetav).
\end{equation}
%
From~\eqref{Eq_ProofSetBintegralbounded} and the fact that $\dot{f}^{-1}$ is continuous and decreasing, there exists a $\lambda \in (0,\infty)$ such that for all $t \in \{s \in \reals : s \geq t_1\}$ constrain in~\eqref{EqEqualToABigOne} is satisfied, which implies that $\set{B} \supseteq [t,\infty)$. This completes the first part of the proof.

%Three cases are considered: $i\bigl)$ $\beta < -\delta^\star_{Q, \dset{z}}$;
%$ii\bigl)$ $\beta > -\delta^\star_{Q, \dset{z}}$; and $iii\bigl)$ $\beta = -\delta^\star_{Q, \dset{z}}$, with $\delta^\star_{Q, \dset{z}}$ in~\eqref{EqDefTStar}.
%
%%
%% Subpart-1 of the Proof part 4 
%%
%In the first case, from the definition of $\delta^\star_{Q, \dset{z}}$ in~\eqref{EqDefTStar}, it follows from~\eqref{EqType2KrescConstrain} that if $\beta < -\delta^\star_{Q, \dset{z}}$, then for all  $\thetav \in \{\thetav \in \supp Q: \foo{L}_{\dset{z}}(\thetav) < -\beta\}$, it holds that
%%
%\begin{subequations}
%\label{EqProofT2Contradict1_all}
%\begin{IEEEeqnarray}{rCl}
%\label{EqProofT2Contradict1}
%	\frac{\diff \Pgibbs[\dset{z}][t]{\bar{P}}{Q}}{\diff Q}(\thetav) 
%	& = & \frac{\lambda}{\foo{L}_{\dset{z}}(\thetav) + \beta} \\
%	& < & 0,
%\end{IEEEeqnarray}
%\end{subequations}
%%
%which contradicts the fact that the function $\frac{\diff \Pgibbs[\dset{z}][t]{\bar{P}}{Q}}{\diff Q}$ in~\eqref{EqGenpdfType2} is nonnegative \cite[Corollary 2.2.2]{ash2000probability}.
%%\cite{Konstantopoulos2011RadNik}).
%%
%The above implies that for all $t \in (0, \infty)$, the function $N_{Q, \dset{z}}$ in~\eqref{EqDefNormFunction} satisfies that $N_{Q, \dset{z}}(t) \not\in (-\infty,-\delta^\star_{Q, \dset{z}})$.
%
%%
%% Subpart-2 of the Proof part 4
%%
%In the second case, if $\beta > -\delta^\star_{Q, \dset{z}}$, it holds that
%\begin{subequations}
%\label{Eq_ProofType2DenLambdaEqV} 
%\begin{IEEEeqnarray}{rCl}
%\label{Eq_ProofType2DenLambdaEqV_s1} 
%	\int \frac{1}{\foo{L}_{\dset{z}}(\thetav) + \beta}\diff Q(\thetav)
%	& \leq & \int \frac{1}{\delta^\star_{Q, \dset{z}}+\beta} \diff Q(\thetav)\\
%	& = &  \frac{1}{\delta^\star_{Q, \dset{z}}+\beta}.\label{Eq_ProofType2DenLambdaEqV_s2}
%\end{IEEEeqnarray}
%\end{subequations}
%%
%Moreover, from~\eqref{Eq_ProofType2DenLambdaEqV} for all $\beta > -\delta^\star_{Q, \dset{z}}$, there exists a $\lambda \in (0,\infty)$ such that the constraint in~\eqref{EqType2KrescConstrainKbarDef} holds, which implies $N^{-1}_{Q, \dset{z}}(\beta) \in (0, \infty)$. 


The second part is as follows.
There are two cases considered under the assumption that $t = t^{\star}_{Q, \dset{z}}$ with $t^{\star}_{Q, \dset{z}}$ defined in~\eqref{EqDefTStar}. 
%
In the first case, if $t^{\star}_{Q, \dset{z}} \in \set{B}$, then it holds that 
%
\begin{subequations}
\label{EqOptProofRNDIntegral}
\begin{IEEEeqnarray}{rCl}
	\int \dot{f}^{-1}(-t^{\star}_{Q, \dset{z}} - \foo{L}_{\dset{z}}(\thetav)) \diff Q(\thetav)
	& < &  \infty,
\end{IEEEeqnarray}
%
which implies that $\set{B} = [t^{\star}_{Q, \dset{z}},\infty)$, with $\set{B}$ defined in~\eqref{EqDefMapNormFunction}. 
In the second case, if $t^{\star}_{Q, \dset{z}} \not\in \set{B}$, then it holds that 
%
\begin{IEEEeqnarray}{rCl}
\label{EqProofT2lowlimDeltaIsLessInfty}
	\int \dot{f}^{-1}(-t^{\star}_{Q, \dset{z}} - \foo{L}_{\dset{z}}(\thetav))\diff Q(\thetav)
	& = & \infty,
	\end{IEEEeqnarray}
\end{subequations}
	  which implies that $\set{B} = (t^{\star}_{Q, \dset{z}},\infty)$, with $\set{B}$ defined in~\eqref{EqDefMapNormFunction}.
%
%Note that the integral is always positive from the fact that for all $\thetav \in \supp Q$, it holds that $\foo{L}_{\dset{z}}(\thetav) > t^{\star}_{Q, \dset{z}}$.
Note that the integral in~\eqref{EqOptProofRNDIntegral} is never zero as it would be a contradiction with~\eqref{EqRiskFunDef}.
%
Hence, from~\eqref{Eq_ProofSetBintegralbounded} and~\eqref{EqOptProofRNDIntegral} the set $\set{B}$ in~\eqref{EqEqualToABigOne} is either the open set $(t^{\star}_{Q, \dset{z}},\infty)$ or the closed set $[t^{\star}_{Q, \dset{z}},\infty)$, which completes the proof.
%--------------------------------------------------End

\end{IEEEproof}
%-----------------------------------------------------
%
% ███████╗███╗░░██╗██████╗░
% ██╔════╝████╗░██║██╔══██╗
% █████╗░░██╔██╗██║██║░░██║
% ██╔══╝░░██║╚████║██║░░██║
% ███████╗██║░╚███║██████╔╝
% ╚══════╝╚═╝░░╚══╝╚═════╝░


%-------------------------------------------------%
%  _
% | |                                   
% | |     ___ _ __ ___  _ __ ___   __ _ 
% | |    / _ \ '_ ` _ \| '_ ` _ \ / _` |
% | |___|  __/ | | | | | | | | | | (_| |
% \_____/\___|_| |_| |_|_| |_| |_|\__,_|
%
%-------------------------------------------------%
%%-------------------------------------------------%
%%        Lemma Type-II Set
%%-------------------------------------------------%
%\begin{lemma}
%\label{lemm_fDR_kset}
%	The set~$\bar{\set{K}}_{Q, \dset{z}}$ in~\eqref{EqDefSetKType2} is either the empty set that satisfies
%	%
%	\begin{subequations}
%	\label{Eq_Type2KsetsubFull}
%	\begin{equation}
%	\label{Eq_Type2Ksetsub}
%		\bar{\set{K}}_{Q, \dset{z}} = (0, \infty).
%	\end{equation}
%	%
%	Moreover, for all $\lambda \in \bar{\set{K}}_{Q, \dset{z}}$ it holds that
%	%
%	\begin{equation}
%	\label{Eq_Type2KConstrain}
%		N_{Q, \dset{z}}(\lambda) \in (-\delta^\star_{Q, \dset{z}}, \infty),
%	\end{equation}
%	\end{subequations}
%	with $N_{Q, \dset{z}}$ defined in~\eqref{EqType2Krescaling}. 
%\end{lemma}
%%
%\begin{IEEEproof}
%	The proof is presented in Appendix~\ref{proof_lemm_fDR_kset}.
%\end{IEEEproof}
%%-------------------------------------------------%


==> Proof_Theo_Type2.tex <==
% !TEX encoding = UTF-8 Unicode
%-------------------------------------------------%   
%   ___                  _____           
%  / _ \                /  ___|          
% / /_\ \_ __  _ ____  _\ `--.  ___  ___ 
% |  _  | '_ \| '_ \ \/ /`--. \/ _ \/ __|
% | | | | |_) | |_) >  </\__/ /  __/ (__ 
% \_| |_/ .__/| .__/_/\_\____/ \___|\___|
%       | |   | |                        
%       |_|   |_|                      
%-------------------------------------------------%
%<*appxsec>
\section{Proof of Lemma~\ref{lemm_Type2RNDbigcirc}}
%
%</appxsec>

%-------------------------------------------------%
% ______                 __ 
% | ___ \               / _|
% | |_/ / __ ___   ___ | |_ 
% |  __/ '__/ _ \ / _ \|  _|
% | |  | | | (_) | (_) | |  
% \_|  |_|  \___/ \___/|_| 
%-------------------------------------------------%
%<*proof>
%--------------
\begin{IEEEproof}
\label{app_lemm_Type2RNDbigcirc}
%
The optimization problem in~\eqref{EqOpType2ERMRERNormal} can be re-written in terms of the Radon-Nikodym derivative of the optimization measure $P$ with respect to the measure $Q$, which yields:
%
\begin{subequations}
\label{EqOpProblemType2fproof}
\begin{IEEEeqnarray}{ccl}
\min_{P \in \bigcirc_{Q}(\set{M})}
&   & \ \int \foo{L}_{\vect{z}}(\thetav)\frac{\diff P}{\diff Q}(\thetav)\, \diff Q(\thetav) \nonumber\\
&   & + \> \lambda \KLlong[\thetav]{Q}{P}, \\
\label{Eq_ProofT2Constraint}
\mathrm{s.t.}  & &  \int \frac{\diff P}{\diff Q}(\thetav)  \diff Q(\thetav) = 1.
\end{IEEEeqnarray}
\end{subequations}
%
The remainder of the proof focuses on the problem in which the optimization is over the function  $\frac{\diff P}{\diff Q}: \set{M} \to \reals$, instead of optimizing the measure $P$. This is due to the fact that for all $P \in \bigcirc_{Q}\left( \set{M} \right)$, the Radon-Nikodym derivate $\frac{\diff P}{\diff Q}$ is unique up to sets of zero measure with respect to $Q$.
%
Let $\mathscr{M}$ be the set of measurable functions $\set{M} \to \reals$ with respect to the measurable spaces $\msblspc{\set{M}}$ and $\left( \reals, \BorSigma{\reals} \right)$ that are absolutely integrable with respect to $Q$.
That is, for all $\hat{g} \in \mathscr{M}$, it holds that
%
\begin{IEEEeqnarray}{rcl}
\label{EqValioLaPena}
\int \abs{ \hat{g} (\vect{\theta})} \diff Q(\vect{\theta}) & < & \infty .
\end{IEEEeqnarray}
 
%
Hence, the optimization problem of interest is:
%
\begin{subequations}
\label{EqOpProblemType2fproof9876}
\begin{IEEEeqnarray}{ccl}
\min_{g \in \mathscr{M}} & &  \int \foo{L}_{\vect{z}}(\thetav) g(\thetav)\, \diff Q(\thetav)- \lambda \int \log(g(\thetav))\diff Q(\thetav) \\
\label{Eq_ProofT2Constraint9876}
\mathrm{s.t.}  & &  \int g(\thetav)  \diff Q(\thetav) = 1.
\end{IEEEeqnarray}
\end{subequations}
%
Let the Lagrangian of the optimization problem in~\eqref{EqOpProblemType2fproof9876} be $L: \mathscr{M}\times \reals \rightarrow \reals$ such that
%
\begin{IEEEeqnarray}{rcl}
\label{EqFunctionalL}\label{EqFunctionalAll}
   L (g, \beta) 
   & = & \int \foo{L}_{\vect{z}}(\thetav)g(\thetav)\, \diff Q(\thetav) - \lambda \int \log(g(\thetav))\, \diff Q(\thetav)  
   \nonumber\\&   & 
   + \> \beta (\int g(\thetav) \, \diff Q(\thetav)-1) \\
   & = & \int \Big( g(\thetav) (\foo{L}_{\vect{z}}(\thetav) + \beta)  - \lambda  \log(g(\thetav)) \Big)  \; \diff Q(\thetav)
   %\nonumber\\&   & 
   - \> \beta,
\end{IEEEeqnarray}
%
where $\beta$ is a  real that acts as a Lagrange multiplier due to the constraint~\eqref{Eq_ProofT2Constraint9876}.
%
Let $\hat{g}: \set{M} \rightarrow \reals$ be a function in $\mathscr{M}$. 
%
The Gateaux differential of the functional $L$ in~\eqref{EqFunctionalAll} at $\left(g, \beta\right) \in \mathscr{M}\times \reals$ in the direction of $\hat{g}$, if it exists, is
%
\begin{IEEEeqnarray}{rcl}
\label{EqNecessaryCondtionType2f}
    \partial L(g, \beta; \hat{g} ) & \triangleq & \left.\frac{\diff}{\diff \gamma}  L(g + \gamma \hat{g}, \beta) \right|_{\gamma = 0}.
\end{IEEEeqnarray}
%
The proof continues under the assumption that the function $g$ and $\hat{g}$ are such that the Gateaux differential in \eqref{EqNecessaryCondtionType2f} exists. Under such an assumption, let the function $r: \reals \rightarrow \reals$ satisfy for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon$ arbitrarily small, that
%
\begin{IEEEeqnarray}{rcl}
\label{EqrType2f}
    r(\gamma) & = & L(g + \gamma \hat{g}, \beta) \\ 
    & = & \int \foo{L}_{\vect{z}}(\thetav)(g (\thetav) + \gamma \hat{g}(\thetav))\, \diff Q(\thetav)
    %\nonumber \\&   &
    - \lambda \int \log(g(\thetav) + \gamma \hat{g}(\thetav))\, \diff Q(\thetav) \nonumber \\    
	&    & + \beta(\int(g(\thetav)  + \gamma \hat{g}(\thetav))\diff Q(\thetav) - 1) \\
	& = & - \beta + \int g (\thetav) ( \foo{L}_{\vect{z}}(\thetav)  + \beta) \diff Q(\thetav)
	%\nonumber\\&   &
	+ \gamma \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta)\diff Q(\thetav) \nonumber\\    
	\label{EqYoLloroCorrigiendoEstaPrueba}
	&    &  + \lambda \int \log(g(\thetav) + \gamma \hat{g}(\thetav))\, \diff Q(\thetav),
\end{IEEEeqnarray}
%
where the last equality is simply an algebraic re-arrangement of terms. From the assumption that the function $g$ and $\hat{g}$ are such that the Gateauz differential in \eqref{EqNecessaryCondtionType2f} exists, it follows that the function $r$ in \eqref{EqrType2f} is differentiable at zero.
%The focus is on the case in which for all  $\gamma \in (-\epsilon, \epsilon)$ and $\epsilon > 0$ arbitrarily small, the inequality $\abs{r(\gamma)} < \infty$ holds. This is essentially due to the fact that  if such a condition does not hold, then, 
%
Note that the first two terms in \eqref{EqYoLloroCorrigiendoEstaPrueba} are independent of $\gamma$; the third term is linear with $\gamma$; and the fourth term can be written using the function $\hat{r}: \reals \to \reals$ such that for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon$ arbitrarily small, satisfies
\begin{IEEEeqnarray}{rcl}
\label{EqrHatForDaunas}
\hat{r}(\gamma) & = &  -\lambda \int \log(g(\thetav) + \gamma \hat{g}(\thetav))\, \diff Q(\thetav).
\end{IEEEeqnarray}
%
Under the same assumption, it follows that the function $\hat{r}$ in \eqref{EqrHatForDaunas} is differentiable at zero. That is, the limit
% so is the function $r$ in \eqref{EqrType2f}, which implies that the  Gateaux differential  $ \partial L(g, \beta; \hat{g}) $ in \eqref{EqNecessaryCondtionType2f} exists.
%
%The objective is to prove that the function $\hat{r}$ is differentiable at zero, which boils down to proving that the limit 
\begin{IEEEeqnarray}{rcl}
\label{EqNeverDoingThisAgain}
\lim_{\delta \to 0}\frac{1}{\delta} ( \hat{r}(\gamma + \delta) - \hat{r}(\gamma) ) 
\end{IEEEeqnarray}
%
exists for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon$ arbitrarily small.
%
The proof of the existence of such a limit relies on the fact that $\log$ is strictly concave and continuous. This implies that $-\log$ is also Lipschitz continuous, which implies that for all $\vect{\theta} \in\set{M}$ and for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon > 0$ arbitrarily small, it holds that
\begin{equation}
\abs{\log(g(\thetav) + \gamma \hat{g}(\thetav)) - \log(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))}  \leq  c \abs{\hat{g}(\thetav) \delta},
%\IEEEeqnarraynumspace
\end{equation}
with $\delta>0$, for some constant $c$ positive and finite, which implies that
\begin{equation}
\label{EqCoffeeTimeIsPast}
\abs{\frac{\log(g(\thetav) + \gamma \hat{g}(\thetav)) - \log(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))}{\delta}} \leq  c \abs{\hat{g}(\thetav)}.
%\IEEEeqnarraynumspace
\end{equation}
%
%
Using these arguments, the limit in \eqref{EqNeverDoingThisAgain} satisfies for all $\gamma  \in (-\epsilon, \epsilon)$, with $\epsilon > 0$ arbitrarily small, that
%
\begin{IEEEeqnarray}{rcl}
%\IEEEeqnarraymulticol{3}{l}{
\lim_{\delta \to 0}\frac{1}{\delta} ( \hat{r}(\gamma + \delta) - \hat{r}(\gamma) ) 
%}\nonumber\\\qquad
& = &\lambda \lim_{\delta \to 0}\frac{1}{\delta} (  \int \log(g(\thetav) + \gamma \hat{g}(\thetav))\, \diff Q(\thetav)\right. \nonumber\\
&   & \left.- \> \int \log(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))\, \diff Q(\thetav)  )\\
& = &\lambda \lim_{\delta \to 0}  \int \frac{\log(g(\thetav) + \gamma \hat{g}(\thetav)) }{\delta} \nonumber\\
&   & - \> \frac{\log(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))}{\delta} \, \diff Q(\thetav) \\
\label{EqTheKeyEqualityOfThisS}
& = & \lambda \int  \frac{\diff }{\diff \gamma}\log(g(\thetav) + \gamma \hat{g}(\thetav))\, \diff Q(\thetav)\\
\label{EqTheKeyEqualityOfThisSh}
& < & \infty,
\end{IEEEeqnarray}
where both the equality in \eqref{EqTheKeyEqualityOfThisS} and the inequality in \eqref{EqTheKeyEqualityOfThisSh} follow from noticing that the conditions for the dominated convergence theorem hold \cite[Theorem~$1.6.9$]{ash2000probability}, namely:
\begin{itemize}
\item For all $\gamma  \in (-\epsilon, \epsilon)$, with $\epsilon > 0$, the inequality in \eqref{EqCoffeeTimeIsPast} holds;
\item The function $\hat{g}$   in \eqref{EqCoffeeTimeIsPast} satisfies the inequality in \eqref{EqValioLaPena}; and 
\item For all $\vect{\theta} \in\set{M}$ and for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon > 0$ arbitrarily small, it holds  that
\begin{IEEEeqnarray}{rcl}
\IEEEeqnarraymulticol{3}{l}{
\lim_{\delta \to 0} \frac{\log(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))   - \log(g(\thetav) + \gamma \hat{g}(\thetav)) }{\delta}
}\nonumber\\\qquad
& = & \> \frac{\mathrm{d}}{\mathrm{d} \gamma} \log(g(\thetav) + \gamma \hat{g}(\thetav)) 
%\IEEEeqnarraynumspace
\\
& = & \>  \frac{\hat{g}(\thetav)}{(g(\thetav) + \gamma \hat{g}(\thetav))},
\end{IEEEeqnarray}
 which follows from the fact that $\log$ is differentiable. 
\end{itemize}

Hence, the derivative of the real function $r$ in \eqref{EqYoLloroCorrigiendoEstaPrueba} is

\begin{IEEEeqnarray}{rcl}
  \frac{\diff}{\diff \gamma}r(\gamma)\,& = & \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta)\diff Q(\thetav)
  %\nonumber\\&   &
  - \lambda \int \frac{\hat{g}(\thetav)}{(g(\thetav) + \gamma \hat{g}(\thetav))} \, \diff Q(\thetav)\\
  \label{EqDerrType2f} & = & \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta \vphantom{\dot{f}} -  \frac{\lambda}{(g(\thetav) + \gamma \hat{g}(\thetav))} )\! \diff Q(\thetav).\IEEEeqnarraynumspace
\end{IEEEeqnarray}
From \eqref{EqNecessaryCondtionType2f} and \eqref{EqDerrType2f}, it follows that
%Gateaux differential $\partial L(g, \beta; \hat{g} )$ in \eqref{EqNecessaryCondtionType2f} exists and  satisfies
%
\begin{IEEEeqnarray}{rcl}
\label{EqGateauxDiffType2f}
	\partial L(g, \beta; \hat{g} )
	%& =& \left.\frac{\diff}{\diff \gamma} r(\gamma) \right|_{\gamma = 0} \\ \label{EqGateauxDiffType2fafa}
	& = & \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta \vphantom{\dot{f}} -  \frac{\lambda}{g(\thetav)} )\! \diff Q(\thetav). 
\end{IEEEeqnarray}
%
The relevance of the Gateaux differential in~\eqref{EqGateauxDiffType2f} stems from \cite[Theorem $1$, page $178$]{luenberger1997bookOptimization}, which unveils the fact that a necessary condition for the functional $L$ in~\eqref{EqFunctionalAll} to have a stationary point at $( \frac{\diff  \Pgibbs{P}{Q}}{\diff Q}, \beta ) \in \set{M} \times [0, \infty)$ is that for all functions $\hat{g} \in \mathscr{M}$,
%
\begin{equation}
\label{EqConditionhiType2f}
\partial L(\frac{\diff \Pgibbs{P}{Q}}{\diff Q}, \beta; \hat{g}) = 0 .
\end{equation}
%
From~\eqref{EqGateauxDiffType2f} and~\eqref{EqConditionhiType2f}, it follows that $\frac{\diff \Pgibbs{P}{Q}}{\diff Q} $ must satisfy for all functions $\hat{g}$ in $\mathscr{M}$ that
%
\begin{equation}
\label{EqIntegralHisZero}
 \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  + \beta  -  \lambda 
 ( \frac{\diff \Pgibbs{P}{Q}}{\diff Q}(\thetav) )^{-1}  ) \diff Q(\thetav) = 0.
\end{equation}
%
This implies that for all $\thetav \in \supp Q$,
%
\begin{equation}
\label{Eq_ProofT2SemiLemma_proof}
\foo{L}_{\vect{z}}(\thetav)  +\beta  -  \lambda  (\frac{\diff \Pgibbs{P}{Q}}{\diff Q}(\thetav)  )^{-1}   = 0,
\end{equation}
%
and thus,
%
\begin{equation}
\label{EqKeyNorthStarx}
  \frac{\diff \Pgibbs{P}{Q}}{\diff Q}(\thetav) = \frac{\lambda}{\beta + \foo{L}_{\dset{z}}(\thetav)},
\end{equation}
%
where $\beta$ is chosen to satisfy \eqref{Eq_ProofT2Constraint9876} and guarantee that for all $\vect{\theta} \in \supp Q$, it holds that $ \frac{\diff \Pgibbs{P}{Q}}{\diff Q}(\thetav) \in (0, \infty)$. That is, 
\begin{equation}
\beta \in \left\lbrace t\in \reals: \forall \vect{\theta} \in \supp Q , 0 < \frac{\lambda}{t + \foo{L}_{\vect{z}}(\thetav)}  \right\rbrace, \text{ and} 
\end{equation}
%
\begin{equation}
1 = \int \frac{\lambda}{\foo{L}_{\dset{z}}(\thetav)+\beta}\diff Q(\thetav).
\end{equation}
which is an assumption of the theorem.

The proof continues by verifying that the measure $\Pgibbs{\bar{P}}{Q}$ that satisfies \eqref{EqKeyNorthStarx} is the unique solution to the optimization problem in \eqref{EqOpProblemType2fproof}. Such verification is done by showing that the objective function in \eqref{EqOpProblemType2fproof} is strictly convex with the optimization variable. Let $P_1$ and $P_2$ be two different probability measures in $\msblspc{\set{M}}$ and let $\alpha$ be in $(0,1)$. Hence,
%
\begin{IEEEeqnarray}{rCl}
\IEEEeqnarraymulticol{3}{l}{
	\foo{R}_{\dset{z}} (\alpha P_1 +(1-\alpha)P_2) + \lambda\KL{\alpha P_1 +(1-\alpha)P_2}{Q}
	}\\
	& = & \foo{R}_{\dset{z}}(\alpha P_1) + \foo{R}_{\dset{z}}((1-\alpha)P_2) + \lambda\KL{\alpha P_1 +(1-\alpha)P_2}{Q}\\
	& > & \foo{R}_{\dset{z}}(\alpha P_1) + \foo{R}_{\dset{z}}((1-\alpha)P_2) + \lambda\KL{\alpha P_1}{Q} + \lambda\KL{(1-\alpha)P_2}{Q}\\
\end{IEEEeqnarray}

where the functional $\foo{R}_{\dset{z}}$ is defined in \eqref{EqRxy}. The equality above follows from the properties of the Lebesgue integral, while the inequality follows from \cite[Theorem 2.2., page ]{InriaRR9454}. This proves that the solution is unique due to the strict concavity of the objective function, which completes the proof.
%Finally, note that the objective function in~\eqref{EqOpProblemType2fproof9876} is the sum of two terms. 
%	%
%	The first one, \ie, $ \int \foo{L}_{\dset{z}}( \thetav )g( \thetav )  \diff Q ( \thetav )$, is linear with $g$.
%	%
%	The second, \ie, $\int -\log (g(\thetav)) \diff Q(\thetav)$, is strictly convex with  $g$ from the assumption that $f$ is strictly convex.
%	%
%	Hence, given that $\lambda>0$, the sum of both terms is strictly convex with  $g$.  This implies the uniqueness of $\Pgibbs{P}{Q}$.	 
\end{IEEEproof}

%</proof>
%-------------------------------------------------%
%
% ███████╗███╗░░██╗██████╗░
% ██╔════╝████╗░██║██╔══██╗
% █████╗░░██╔██╗██║██║░░██║
% ██╔══╝░░██║╚████║██║░░██║
% ███████╗██║░╚███║██████╔╝
% ╚══════╝╚═╝░░╚══╝╚═════╝░


%-------------------------------------------------%
% _
%| |                                   
%| |     ___ _ __ ___  _ __ ___   __ _ 
%| |    / _ \ '_ ` _ \| '_ ` _ \ / _` |
%| |___|  __/ | | | | | | | | | | (_| |
%\_____/\___|_| |_| |_|_| |_| |_|\__,_|
%
%-------------------------------------------------%
%       Lemma Radon Nikodym Derivative Mutual
%-------------------------------------------------%
%\begin{lemma}
%\label{lemm_Type2RNDbigcirc}
%For all $\lambda \in \bar{\set{K}}_{Q, \dset{z}}$, the solution to the optimization problem in~\eqref{EqOpType2ERMRERancillary} is the unique probability measure $\Pgibbs{\bar{P}}{Q}$ in~\eqref{EqGenpdfType2}.
%\end{lemma}
%\begin{IEEEproof}
%	The proof is presented in Appendix~\ref{app_lemm_Type2RNDbigcirc}.
%\end{IEEEproof}
%-------------------------------------------------%


==> Proof_Theo_fDivRN_IEEEtran.tex <==
% !TEX encoding = UTF-8 Unicode
%-------------------------------------------------%   
%   ___                  _____           
%  / _ \                /  ___|          
% / /_\ \_ __  _ ____  _\ `--.  ___  ___ 
% |  _  | '_ \| '_ \ \/ /`--. \/ _ \/ __|
% | | | | |_) | |_) >  </\__/ /  __/ (__ 
% \_| |_/ .__/| .__/_/\_\____/ \___|\___|
%       | |   | |                        
%       |_|   |_|                      
%-------------------------------------------------%
%<*appxsec>
\section{Proof of Theorem~\ref{Theo_f_ERMRadNik}}
%
%</appxsec>

%-------------------------------------------------%
% ______                 __ 
% | ___ \               / _|
% | |_/ / __ ___   ___ | |_ 
% |  __/ '__/ _ \ / _ \|  _|
% | |  | | | (_) | (_) | |  
% \_|  |_|  \___/ \___/|_| 
%-------------------------------------------------%
%<*proof>
%--------------
\begin{IEEEproof}
\label{app_theo_f_ERMRadNik}
%
The optimization problem in~\eqref{EqOp_f_ERMRERNormal} can be re-written in terms of the Radon-Nikodym derivative of the optimization measure $P$ with respect to the measure $Q$, which yields
%
\begin{subequations}
\label{EqOpProblemType2fproof}
\begin{IEEEeqnarray}{ccl}
\min_{P \in \bigtriangleup_{Q}\left( \set{M} \right) } 
&   & \ \int \foo{L}_{\vect{z}}(\thetav)\frac{\diff P}{\diff Q}(\thetav)\,\diff Q(\thetav) \nonumber \\
&   & + \> \lambda \int f(\frac{\diff P}{\diff Q}(\thetav))\diff Q(\thetav)\\
\label{Eq_ProofT2Constraint}
\mathrm{s.t.}  & &  \int \frac{\diff P}{\diff Q}(\thetav)  \diff Q(\thetav) = 1.
\end{IEEEeqnarray}
\end{subequations}
%
The remainder of the proof focuses on the problem in which the optimization is over the function  $\frac{\diff P}{\diff Q}: \set{M} \to [0, \infty)$, which represents the Radon-Nikodym derivate of $P$ with respect to $Q$. Hence, instead of optimizing the measure $P$, the optimization is over the function $\frac{\diff P}{\diff Q}$. This is due to the fact that for all $P \in \bigtriangleup_{Q}\left( \set{M} \right)$, the Radon-Nikodym derivate $\frac{\diff P}{\diff Q}$ is unique up to sets of zero measure with respect to $Q$.
%
Let $\mathscr{M}$ be the set of measurable functions $\set{M} \to \reals$ with respect to the measurable spaces $\msblspc{\set{M}}$ and $\left( \reals, \BorSigma{\reals} \right)$ that are absolutely integrable with respect to $Q$.
That is, for all $\hat{g} \in \mathscr{M}$, it holds that
%
\begin{IEEEeqnarray}{rcl}
\label{EqValioLaPena}
\int \abs{ \hat{g} (\vect{\theta})} \diff Q(\vect{\theta}) & < & \infty.
\end{IEEEeqnarray}
%
Hence, the optimization problem of interest is
%
\begin{subequations}
\label{EqOpProblemType2fproof9876}
\begin{IEEEeqnarray}{ccl}
\min_{g \in \mathscr{M}} & &  \int \foo{L}_{\vect{z}}(\thetav) g(\thetav)\,\diff Q(\thetav)+ \lambda \int f(g(\thetav))\diff Q(\thetav) \\
\label{Eq_ProofT2Constraint9876}
\mathrm{s.t.}  & &  \int g(\thetav)  \diff Q(\thetav) = 1.
\end{IEEEeqnarray}
\end{subequations}
%
Let the Lagrangian of the optimization problem in~\eqref{EqOpProblemType2fproof9876} be $L: \mathscr{M}\times \reals \rightarrow \reals$ such that
%
\begin{IEEEeqnarray}{rcl}
\label{EqFunctionalL}\label{EqFunctionalAll}
   L (g,\beta) 
   & = & \int \foo{L}_{\vect{z}}(\thetav)g(\thetav)\,\diff Q(\thetav)+ \lambda \int f(g(\thetav))\,\diff Q(\thetav)  \nonumber \\
   &   & + \> \beta (\int g(\thetav) \,\diff Q(\thetav)-1), \\
   & = & \int \Big( g(\thetav) (\foo{L}_{\vect{z}}(\thetav) + \beta)  + \lambda  f(g(\thetav)) \Big)  \; \diff Q(\thetav) \nonumber\\
   &   & - \>\beta, \IEEEeqnarraynumspace
\end{IEEEeqnarray}
%
where $\beta$ is a  real that acts as a Lagrange multiplier due to the constraint~\eqref{Eq_ProofT2Constraint9876}.
%
Let $\hat{g}: \set{M} \rightarrow \reals$ be a function in $\mathscr{M}$. 
%
The Gateaux differential of the functional $L$ in~\eqref{EqFunctionalAll} at $\left(g, \beta\right) \in \mathscr{M}\times \reals$ in the direction of $\hat{g}$, if it exists, is
%
\begin{IEEEeqnarray}{rcl}
\label{EqNecessaryCondtionType2f}
    \partial L(g, \beta; \hat{g} ) & \triangleq & \left.\frac{\diff}{\diff \gamma}  L(g + \gamma \hat{g}, \beta) \right|_{\gamma = 0}.
\end{IEEEeqnarray}
%
The proof continues under the assumption that the function $g$ and $\hat{g}$ are such that the Gateaux differential in~\eqref{EqNecessaryCondtionType2f} exists. Under such an assumption, let the function $r: \reals \rightarrow \reals$ satisfy for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon$ arbitrarily small, that
%
\begin{IEEEeqnarray}{rcl}
\label{EqrType2f}
    r(\gamma) & = & L(g + \gamma \hat{g}, \beta) \\ 
\nonumber
    & = & \int \foo{L}_{\vect{z}}(\thetav)(g (\thetav) + \gamma \hat{g}(\thetav))\,\diff Q(\thetav) \nonumber\\
    &   & + \> \lambda \int f(g(\thetav) + \gamma \hat{g}(\thetav))\,\diff Q(\thetav) \nonumber \\    
	&   & + \> \beta(\int(g(\thetav)  + \gamma \hat{g}(\thetav))\diff Q(\thetav) - 1) \\ 
	& = & \int g (\thetav) ( \foo{L}_{\vect{z}}(\thetav)  + \beta) \diff Q(\thetav) \nonumber \\
	&   & + \> \gamma \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta)\diff Q(\thetav) - \beta \nonumber\\
	&    &  + \lambda \int f(g(\thetav) + \gamma \hat{g}(\thetav))\,\diff Q(\thetav),\label{EqYoLloroCorrigiendoEstaPrueba}
\end{IEEEeqnarray}
%
where the last equality is simply an algebraic re-arrangement of terms. From the assumption that the function $g$ and $\hat{g}$ are such that the Gateauz differential in~\eqref{EqNecessaryCondtionType2f} exists, it follows that the function $r$ in~\eqref{EqrType2f} is differentiable at zero.
%The focus is on the case in which for all  $\gamma \in (-\epsilon, \epsilon)$ and $\epsilon > 0$ arbitrarily small, the inequality $\abs{r(\gamma)} < \infty$ holds. This is essentially due to the fact that  if such a condition does not hold, then, 
%
Note that the first two terms in~\eqref{EqYoLloroCorrigiendoEstaPrueba} are independent of $\gamma$; the third term is linear with $\gamma$; and the fourth term can be written using the function $\hat{r}: \reals \to \reals$ such that for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon$ arbitrarily small, it holds that
\begin{IEEEeqnarray}{rcl}
\label{EqrHatForDaunas}
\hat{r}(\gamma) & = &  \lambda \int f(g(\thetav) + \gamma \hat{g}(\thetav))\,\diff Q(\thetav) .
\end{IEEEeqnarray}
%
Under the same assumption, it follows that the function $\hat{r}$ in~\eqref{EqrHatForDaunas} is differentiable at zero. That is, the limit
% so is the function $r$ in~\eqref{EqrType2f}, which implies that the  Gateaux differential  $ \partial L(g, \beta; \hat{g}) $ in~\eqref{EqNecessaryCondtionType2f} exists.
%
%The objective is to prove that the function $\hat{r}$ is differentiable at zero, which boils down to proving that the limit 
\begin{IEEEeqnarray}{rcl}
\label{EqNeverDoingThisAgain}
\lim_{\delta \to 0}\frac{1}{\delta} ( \hat{r}(\gamma + \delta) - \hat{r}(\gamma) ) 
\end{IEEEeqnarray}
%
exists for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon$ arbitrarily small.
%
The proof of the existence of such a limit relies on the fact that $f$ is strictly convex and continuous. This implies that $f$ is Lipschitz continuous, which implies that for all $\vect{\theta} \in\set{M}$ and for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon > 0$ arbitrarily small, it holds that
\begin{equation}
\abs{f(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))   - f(g(\thetav) + \gamma \hat{g}(\thetav))}  \leq  c \abs{\hat{g}(\thetav)} \abs{\delta},
\end{equation}
for some constant $c$ positive and finite, which implies that
\begin{equation}
\label{EqCoffeeTimeIsPast}
\abs{\frac{f(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))   - f(g(\thetav) + \gamma \hat{g}(\thetav))}{\delta}}  \leq   c \abs{\hat{g}(\thetav)}.
\end{equation}
%
%
Using these arguments, the limit in~\eqref{EqNeverDoingThisAgain} satisfies for all $\gamma  \in (-\epsilon, \epsilon)$, with $\epsilon > 0$ arbitrarily small, that
%
\begin{IEEEeqnarray}{rcl}
\IEEEeqnarraymulticol{3}{l}{ 
\lim_{\delta \to 0}\frac{1}{\delta} ( \hat{r}(\gamma + \delta) - \hat{r}(\gamma) )
}\nonumber \\
& = &\lambda \lim_{\delta \to 0}\frac{1}{\delta} (  \int f(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))\,\diff Q(\thetav) \right.\nonumber \\
&   & \left. - \>  \int f(g(\thetav) + \gamma \hat{g}(\thetav))\,\diff Q(\thetav) )\\
& = & \lambda \lim_{\delta \to 0}  \int (\frac{f(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav)) }{\delta} \right. \nonumber \\
&   & \left. - \> \frac{f(g(\thetav) + \gamma \hat{g}(\thetav)) }{\delta}) \,\diff Q(\thetav) \\
\label{EqTheKeyEqualityOfThisS}
& = & \lambda \int  \dot{f}(g(\thetav) + \gamma \hat{g}(\thetav))  \hat{g}(\thetav)\,\diff Q(\thetav)\\
\label{EqTheKeyEqualityOfThisSh}
& < & \infty,
\end{IEEEeqnarray}
where both the equality in~\eqref{EqTheKeyEqualityOfThisS} and the inequality in~\eqref{EqTheKeyEqualityOfThisSh} follow from noticing that the conditions for the dominated convergence theorem hold \cite[Theorem~$1.6.9$]{ash2000probability}, namely:
\begin{itemize}
\item For all $\gamma  \in (-\epsilon, \epsilon)$, with $\epsilon > 0$, the inequality in~\eqref{EqCoffeeTimeIsPast} holds;
\item The function $\hat{g}$   in~\eqref{EqCoffeeTimeIsPast} satisfies the inequality in~\eqref{EqValioLaPena}; and 
\item For all $\vect{\theta} \in\set{M}$ and for all $\gamma \in (-\epsilon, \epsilon)$, with $\epsilon > 0$ arbitrarily small, it holds  that
\begin{IEEEeqnarray}{rcl}
\IEEEeqnarraymulticol{3}{l}{
\lim_{\delta \to 0} \frac{f(g(\thetav) + (\gamma + \delta) \hat{g}(\thetav))   - f(g(\thetav) + \gamma \hat{g}(\thetav)) }{\delta}
}\nonumber\\\qquad
& = & \> \frac{\mathrm{d}}{\mathrm{d} \gamma} f(g(\thetav) + \gamma \hat{g}(\thetav)) 
%\IEEEeqnarraynumspace
\\
& = & \>  \dot{f}(g(\thetav) + \gamma \hat{g}(\thetav)),
\end{IEEEeqnarray}
which follows from the fact that $f$ is differentiable. 
\end{itemize}
%
Hence, the derivative of the real function $r$ in~\eqref{EqYoLloroCorrigiendoEstaPrueba} is
\begin{IEEEeqnarray}{rcl}
\IEEEeqnarraymulticol{3}{l}{\frac{\diff}{\diff \gamma}r(\gamma)}\nonumber\\
& = & \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta)\diff Q(\thetav) \nonumber \\
&   & + \>  \lambda \int  \dot{f}(g(\thetav) + \gamma \hat{g}(\thetav))  \hat{g}(\thetav)\,\diff Q(\thetav)\\
\label{EqDerrType2f}
& = & \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta  +  \lambda  \dot{f}(g(\thetav) + \gamma \hat{g}(\thetav))  ) \diff Q(\thetav).
\end{IEEEeqnarray}
From~\eqref{EqNecessaryCondtionType2f} and~\eqref{EqDerrType2f}, it follows that
%
\begin{IEEEeqnarray}{rcl}
	\label{EqGateauxDiffType2f}
	\!\!\!\! \partial L(g, \beta; \hat{g} ) 
	& = &  \left.\frac{\diff}{\diff \gamma} r(\gamma) \right|_{\gamma = 0}\qquad \qquad \qquad \qquad \qquad \qquad \\
	\label{EqGateauxDiffType2fafa}
	& = & \!\int\!\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta  +  \lambda  \dot{f}(g(\thetav)  )  ) \diff Q(\thetav). 
\end{IEEEeqnarray}
%
The relevance of the Gateaux differential in~\eqref{EqGateauxDiffType2f} stems from \cite[Theorem $1$]{luenberger1997bookOptimization}, which unveils the fact that a necessary condition for the functional $L$ in~\eqref{EqFunctionalAll} to have a stationary point at $( \frac{\diff  \Pgibbs{P}{Q}}{\diff Q}, \beta ) \in \set{M} \times [0, \infty)$ is that for all functions $\hat{g} \in \mathscr{M}$,
%
\begin{equation}
\label{EqConditionhiType2f}
\partial L(\frac{\diff \Pgibbs{P}{Q}}{\diff Q}, \beta; \hat{g}) = 0.
\end{equation}
%
From~\eqref{EqGateauxDiffType2fafa} and~\eqref{EqConditionhiType2f}, it follows that $\frac{\diff \Pgibbs{P}{Q}}{\diff Q} $ must satisfy for all functions $\hat{g}$ in $\mathscr{M}$ that
%
\begin{equation}
\label{EqIntegralHisZero}
 \int\hat{g}(\thetav)(\foo{L}_{\vect{z}}(\thetav)  +\beta  +  \lambda  \dot{f}(\frac{\diff \Pgibbs{P}{Q}}{\diff Q}(\thetav)  )  ) \diff Q(\thetav) = 0.
\end{equation}
%
This implies that for all $\thetav \in \supp Q$,
%
\begin{equation}
\label{Eq_ProofT2SemiLemma_proof}
\foo{L}_{\vect{z}}(\thetav)  +\beta  +  \lambda  \dot{f}(\frac{\diff \Pgibbs{P}{Q}}{\diff Q}(\thetav)  )   = 0,
\end{equation}
%
and thus,
%
\begin{equation}
\label{EqKeyNorthStarx}
  \frac{\diff \Pgibbs{P}{Q}}{\diff Q}(\thetav) = \dot{f}^{-1}(-\frac{\beta + \foo{L}_{\dset{z}}(\thetav)}{\lambda}),
\end{equation}
%
where $\beta$ is chosen to satisfy~\eqref{EqEqualToABigOne} and guarantee that for all $\vect{\theta} \in \supp Q$, it holds that $ \dot{f}^{-1}(-\frac{\beta + \foo{L}_{\dset{z}}(\thetav)}{\lambda}) \in (0, \infty)$. That is, 
\begin{equation}
\beta \in \left\lbrace t\in \reals: \forall \vect{\theta} \in \supp Q , 0 <  \dot{f}^{-1} \left( -\frac{t + \foo{L}_{\vect{z}}(\thetav)}{\lambda} \right)\right\rbrace, 
\end{equation}
which is an assumption of the theorem.

%The proof continues by verifying that the measure $\Pgibbs{P}{Q}$ that satisfies~\eqref{EqKeyNorthStarx} is the unique solution to the optimization problem in~\eqref{EqOpProblemType2fproof}. Such verification is done by showing that the objective function in~\eqref{EqOpProblemType2fproof} is strictly convex with the optimization variable. Let $P_1$ and $P_2$ be two different probability measures in $\msblspc{\set{M}}$ and let $\alpha$ be in $(0,1)$. Hence,
%%
%\begin{IEEEeqnarray}{rCl}
%\IEEEeqnarraymulticol{3}{l}{
%	\foo{R}_{\dset{z}} (\alpha P_1 +(1-\alpha)P_2) + \lambda\KL{\alpha P_1 +(1-\alpha)P_2}{Q}
%	}\nonumber\\
%	& = & \foo{R}_{\dset{z}}(\alpha P_1) + \foo{R}_{\dset{z}}((1-\alpha)P_2) \nonumber\\
%	&   & + \lambda\KL{\alpha P_1 +(1-\alpha)P_2}{Q}\\
%	& > & \foo{R}_{\dset{z}}(\alpha P_1) + \foo{R}_{\dset{z}}((1-\alpha)P_2) + \lambda\KL{\alpha P_1}{Q} \nonumber \\
%	&   &+ \lambda\KL{(1-\alpha)P_2}{Q} \label{EqProofTheoIneConvexDiv}
%\end{IEEEeqnarray}
%
Finally, note that the objective function in~\eqref{EqOpProblemType2fproof9876} is the sum of two terms. 
	%
	The first one, \ie, $ \int \foo{L}_{\dset{z}}( \thetav )g( \thetav )  \diff Q ( \thetav )$, is linear with $g$.
	%
	The second, \ie, $\int -\log (g(\thetav)) \diff Q(\thetav)$, is strictly convex with  $g$ from the assumption that $f$ is strictly convex.
	%
	Hence, given that $\lambda>0$, the sum of both terms is strictly convex with  $g$.
	%
	This implies the uniqueness of $\Pgibbs{P}{Q}$, which completes the proof.	 
\end{IEEEproof}

%</proof>
%-------------------------------------------------%
%
% ███████╗███╗░░██╗██████╗░
% ██╔════╝████╗░██║██╔══██╗
% █████╗░░██╔██╗██║██║░░██║
% ██╔══╝░░██║╚████║██║░░██║
% ███████╗██║░╚███║██████╔╝
% ╚══════╝╚═╝░░╚══╝╚═════╝░


%-------------------------------------------------%
% _
%| |                                   
%| |     ___ _ __ ___  _ __ ___   __ _ 
%| |    / _ \ '_ ` _ \| '_ ` _ \ / _` |
%| |___|  __/ | | | | | | | | | | (_| |
%\_____/\___|_| |_| |_|_| |_| |_|\__,_|
%
%-------------------------------------------------%
%       Lemma Radon Nikodym Derivative Mutual
%-------------------------------------------------%
%\begin{lemma}
%\label{lemm_Type2RNDbigcirc}
%For all $\lambda \in \bar{\set{K}}_{Q, \dset{z}}$, the solution to the optimization problem in~\eqref{EqOpType2ERMRERancillary} is the unique probability measure $\Pgibbs{P}{Q}$ in~\eqref{EqGenpdffDv}.
%\end{lemma}
%\begin{IEEEproof}
%	The proof is presented in Appendix~\ref{app_lemm_Type2RNDbigcirc}.
%\end{IEEEproof}
%-------------------------------------------------%
